Decentralized and Asymmetric Multi-Agent Learning in Construction Sites

Multi-agent collaboration involves multiple participants working together in a shared environment to achieve a common goal. These agents share information, divide tasks, and synchronize their actions. Key aspects of multi agent collaboration include coordination, communication, task allocation, cooperation, adaptation, and decentralization. On construction sites, surface grading is the process of leveling sand piles to increase a specific area's height. In this scenario, a bulldozer grades while a dumper allocates sand piles. Our work aims to utilize a multi-agent approach to enable these vehicles to collaborate effectively. To this end, we propose a decentralized and asymmetric multi-agent learning approach for construction sites (DAMALCS). We formulate DAMALCS to reduce expected collisions for operating vehicles. Therefore, we develop two heuristic experts capable of achieving their joint goal optimally by applying an innovative prioritization method. In this approach, the bulldozer's movements take precedence over the dumper's operations, enabling the bulldozer to clear the path for the dumper and ensure continuous operation of both vehicles. Since heuristics alone are insufficient in real-world scenarios, we utilize them to train AI agents, which proves to be highly effective. We simultaneously train the bulldozer and dumper agents to operate within the same environment, aiming to avoid collisions and optimize performance in terms of time efficiency and sand volume handling. Our trained agents and heuristics are evaluated in both simulation and real-world lab experiments, testing them under various conditions, such as visual noise and localization errors. The results demonstrate that our approach significantly reduces collision rates for these vehicles.

==> 09-bio_notes.tex <==
%\section{BIO} \label{sec:bio_notes} 

\bibliographystyle{IEEEtran}
\bibliography{export}
% biography section
\vskip -2\baselineskip plus -1fil



\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio_images/Yakov_image1.jpg}}]{Yakov Miron}
(Member IEEE) Received B.Sc degree in Electrical Engineering from Beer-Sheva University, Israel in 2009 and M.Sc. degree in Electrical Engineering from Tel-Aviv University in 2016, Israel. He is currently a senior manager and senior research scientist at Bosch Research and pursuing an Ph.D. degree with the Autonomous Navigation and Sensor Fusion Laboratory, the Hatter Department of Marine Technologies, University of Haifa, Israel. His research interests include Perception, Navigation, and Path Planning for mobile robots and autonomous driving.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio_images/dan_bio.jpg}}]{Dan Navon}
Received his B.Sc. and M.Sc. degrees in Computer Science from Technion - Israel Institute of Technology in 2018, 2023, respectively.
He is currently an algorithm developer at Adasky, where he works on perception tasks for autonomous driving.
His research interests include perception, SLAM, and vision-aided navigation for mobile platforms.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio_images/Yuval_image.jpg}}]{Yuval Goldfracht}
Received B.Sc degree in Electrical Engineering from the Technion, Israel in 2016 and M.Sc. degree in Marine Technologies from the University of Haifa, Israel in 2018. He is currently a research engineer at Bosch Research. His research interests include Perception, Navigation, and Path Planning for mobile robots.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio_images/dotan_image.jpg}}]{Dotan Di~Castro}
Received his B.Sc. M.Sc. and Ph.D. degrees in Electrical Engineering from Technion, Israel Institute of Technology in 2003, 2006, and 2010 respectively. He is currently a lab and group manager and research scientist at Bosch Center for AI in Haifa, Israel. His research interests are computer vision and reinforcement learning, as well as robotics and autonomous systems. Prior to Bosch he was a senior research scientist at Yahoo! research and worked for several startups.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio_images/Itzik_image.jpeg}}]
{Itzik Klein} (Senior Member, IEEE) Received B.Sc. and M.Sc. degrees in Aerospace Engineering from the Technion - Israel Institute of Technology, Haifa, Israel, in 2004 and 2007, respectively, and a Ph.D. degree in Geo-information Engineering from the Technion - Israel Institute of Technology, in 2011. He is Associate Professor, heading the Autonomous Navigation and Sensor Fusion Lab, at the Charney School of Marine Sciences, Hatter Department of Marine Technologies, University of Haifa. He is an IEEE Senior Member and member of the Editorial Board of the IEEE Journal of Indoor and Seamless Positioning and Navigation (J-ISPIN). He is Distinguished Lecturer for the IEEE Oceanic Engineering Society. Before joining the University of Haifa, he worked for more than 15 years at leading companies in Israel on navigation topics. He has a wide range of experience in navigation systems and sensor fusion from both industry and academic perspectives. His research interests lie in the intersection of artificial intelligence with inertial sensing, sensor fusion, and robotics.
\end{IEEEbiography}




